Model Order Reduction of Combustion Processes with Complex Front Dynamics

In this work we present a data driven method, used to improve mode-based model order reduction of transport fields with sharp fronts. We assume that the original flow field $q(\mathbf{x},t)=f(\phi(\mathbf{x},t))$ can be reconstructed by a front shape function $f$ and a level set function $\phi$. The level set function is used to generate a local coordinate, which parametrizes the distance to the front. In this way, we are able to embed the local 1D description of the front for complex 2D front dynamics with merging or splitting fronts, while seeking a low rank description of $\phi$. Here, the freedom of choosing $\phi$ far away from the front can be used to find a low rank description of $\phi$ which accelerates the convergence of $\Vert q- f(\phi_n)\Vert$, when truncating $\phi$ after the $n$th mode. We demonstrate the ability of this new ansatz for a 2D propagating flame with a moving front.

==> arxiv_version/images/tikz/L2error1.tex <==
% This file was created by matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
\definecolor{mycolor3}{rgb}{0.92900,0.69400,0.12500}%
%
\begin{tikzpicture}

\begin{axis}[%
width=0.98\figurewidth,
height=\figureheight,
at={(0\figurewidth,0\figureheight)},
scale only axis,
xmin=0,
xmax=35,
xlabel style={font=\color{white!15!black}},
xlabel={$n$ modes},
ymode=log,
ymin=1e-05,
ymax=1,
yminorticks=true,
ylabel style={font=\color{white!15!black}},
ylabel={relative error},
axis background/.style={fill=white},
legend style={legend cell align=left, align=left, fill=none, draw=none},
scaled ticks=false, xticklabel style={/pgf/number format/fixed},yticklabel style={/pgf/number format/fixed}
]
\addplot [color=mycolor1, mark=+, mark options={solid, mycolor1}]
  table[row sep=crcr]{%
0	1\\
1	0.208229443543112\\
2	0.102534111517672\\
3	0.0684607934553688\\
4	0.0525537994592058\\
5	0.0390562664701335\\
6	0.0314835452029856\\
7	0.0269628292186073\\
8	0.0219475880704862\\
9	0.0188429414737321\\
10	0.0163972664662912\\
11	0.013965614250307\\
12	0.0125463122580134\\
13	0.0109721803712042\\
14	0.00955260974393814\\
15	0.00883978008328678\\
16	0.00751239333211285\\
17	0.00653701996177867\\
18	0.00619338004598776\\
19	0.00522964408485424\\
20	0.00480151486331356\\
21	0.00442394922096749\\
22	0.00381990100342253\\
23	0.00353175709993112\\
24	0.00322741659242932\\
25	0.00284387635092358\\
26	0.00259873041169349\\
27	0.00242590484263579\\
28	0.00222875988078201\\
29	0.00221177107765771\\
30	0.0018469066254779\\
31	0.00169378260522157\\
32	0.00118759149876739\\
33	0.00106989788831319\\
34	0.000736697540171317\\
35	0.000718134579281819\\
36	0.000686160746658145\\
37	0.000402244487173694\\
38	0.00035469526584975\\
};
\addlegendentry{$\Vert q-q_n\Vert_2/\Vert q\Vert_2$}

\addplot [color=mycolor2, mark=x, mark options={solid, mycolor2}]
  table[row sep=crcr]{%
0	1\\
1	0.265510800527437\\
2	0.0463614181640376\\
3	0.0283715884758292\\
4	0.0199029658072694\\
5	0.0126201418660051\\
6	0.0118068407836256\\
7	0.00922624224162863\\
8	0.00722770731927204\\
9	0.00580362197791494\\
10	0.00468439293661942\\
11	0.00452342661533994\\
12	0.00362688541669926\\
13	0.00357160680174792\\
14	0.00352620886483618\\
15	0.003414557436661\\
16	0.00336364279101439\\
17	0.00333974173521294\\
18	0.00325883933378627\\
19	0.00323821649124755\\
20	0.00323636312864429\\
21	0.00323328260047271\\
22	0.00323555684310697\\
23	0.00323525501204207\\
24	0.00323540938117981\\
25	0.00323492470907774\\
26	0.0032351082490826\\
27	0.00323499042213585\\
28	0.00323481579946083\\
29	0.00323483255312862\\
30	0.00323472085101366\\
31	0.00323470372267496\\
32	0.0032347178590847\\
33	0.00323472310833984\\
34	0.00323470720702309\\
35	0.0032347257942111\\
36	0.00323474819740701\\
37	0.00323475213020157\\
38	0.0032347349939891\\
39	0.00323474067829452\\
};
\addlegendentry{$\Vert q-f(\phi_n)\Vert_2/\Vert q\Vert_2$}

\addplot [color=mycolor3, mark=o, mark options={solid, mycolor3}]
  table[row sep=crcr]{%
0	1\\
1	0.204567953291119\\
2	0.0443917947230602\\
3	0.0232309619741152\\
4	0.0085709403775077\\
5	0.00731862287415803\\
6	0.00489921557644142\\
7	0.00283262683278337\\
8	0.00178617558199724\\
9	0.00164870807510567\\
10	0.00120265155748921\\
11	0.00111233314508517\\
12	0.000823138940726148\\
13	0.000677207015357723\\
14	0.000553609434910426\\
15	0.000528998406168389\\
16	0.00045021550101092\\
17	0.000379150226217814\\
18	0.000338482402789455\\
19	0.000280990340105079\\
20	0.000254682920176477\\
21	0.000242397249647828\\
22	0.000218394872009236\\
23	0.000207289773748153\\
24	0.00016621041992349\\
25	0.000154863734452438\\
26	0.000120363422383624\\
27	0.000109332163294977\\
28	8.97499587945491e-05\\
29	8.94511649719974e-05\\
30	8.04497242724231e-05\\
31	7.50541169400655e-05\\
32	7.2479741508773e-05\\
33	6.90021502406033e-05\\
34	6.22861791475555e-05\\
35	6.12830318216549e-05\\
36	5.66541279019915e-05\\
37	5.29509644899316e-05\\
38	4.88074401371284e-05\\
};
\addlegendentry{$\Vert\phi-\phi_n\Vert_2/\Vert\phi\Vert_2$}

\addplot [color=black, dashed, line width=2.0pt, forget plot]
  table[row sep=crcr]{%
1	0.00323473166550014\\
39	0.00323473166550014\\
};
\node[right, align=left]
at (axis cs:2,0.002) {$\Delta f$};
\end{axis}
\end{tikzpicture}%

==> arxiv_version/images/tikz/levelset1Dsigma.tex <==
% This file was created by matplotlib2tikz v0.7.4.
\begin{tikzpicture}

\definecolor{color0}{rgb}{1,0.647058823529412,0}

\begin{axis}[
height=\figureheight,
legend cell align={left},
legend style={at={(0.5,0.6)}, anchor=north, draw=none},
log basis y={10},
tick align=outside,
tick pos=left,
title={${\sigma_n(X)}/{\Vert X\Vert_2}$},
width=\figurewidth,
x grid style={white!69.01960784313725!black},
xlabel={Mode \(\displaystyle n\)},
xmajorgrids,
xmin=0, xmax=20,
xminorgrids,
xtick style={color=black},
y grid style={white!69.01960784313725!black},
ymajorgrids,
ymin=4.54213436950621e-18, ymax=6.69645204306777,
yminorgrids,
ymode=log,
ytick style={color=black}
]
\addplot [blue, mark=*, mark size=1, mark options={solid}]
table {%
0 1
1 0.333307703774789
2 0.199954027121491
3 0.142791811095647
4 0.111027012985494
5 0.0908068272042107
6 0.0768032340419105
7 0.0665299577867899
8 0.0586707576941898
9 0.0524636522024691
10 0.0474369849968113
11 0.0432831983625682
12 0.0397931956823475
13 0.0368198763784882
14 0.0342567600498823
15 0.0320248853257144
16 0.0300644729534269
17 0.0283294474291522
18 0.0267837355609547
19 0.0253987040912931
20 0.0241513474298762
21 0.0230229812714542
22 0.0219982847067642
23 0.0210645870127596
24 0.020211329204153
25 0.0194296523606727
26 0.0187120792278299
27 0.0180522653322048
28 0.0174448025186014
29 0.0168850624490217
30 0.0163690708692308
31 0.0158934057818367
32 0.0154551143525037
33 0.0150516446111154
34 0.0146807889238899
35 0.014340636896266
36 0.0140295358836925
37 0.013746057681911
38 0.0134889702748358
39 0.0132572135707566
40 0.0130498795780921
41 0.0128661931241879
42 0.0127054977392726
43 0.0125672391273757
44 0.0124514240610197
45 0.0123563603073238
46 0.0122830307689976
47 0.0122308092701341
48 0.0121995376914025
49 0.00557113083247043
};
\addlegendentry{$X^q_{ij}=q(x_i,t_j)$}
\addplot [color0, dashed, mark=triangle*, mark size=1, mark options={solid,rotate=90}]
table {%
0 1
1 0.983468842746643
2 2.98409190362933e-16
3 2.39087578108502e-16
4 1.71640175526394e-16
5 1.06455300209217e-16
6 9.95076345691556e-17
7 9.95076345691556e-17
8 9.95076345691556e-17
9 9.95076345691556e-17
10 9.95076345691556e-17
11 9.95076345691556e-17
12 9.95076345691556e-17
13 9.95076345691556e-17
14 9.95076345691556e-17
15 9.95076345691556e-17
16 9.95076345691556e-17
17 9.95076345691556e-17
18 9.95076345691556e-17
19 9.95076345691556e-17
20 9.95076345691556e-17
21 9.95076345691556e-17
22 9.95076345691556e-17
23 9.95076345691556e-17
24 9.95076345691556e-17
25 9.95076345691556e-17
26 9.95076345691556e-17
27 9.95076345691556e-17
28 9.95076345691556e-17
29 9.95076345691556e-17
30 9.95076345691556e-17
31 9.95076345691556e-17
32 9.95076345691556e-17
33 9.95076345691556e-17
34 9.95076345691556e-17
35 9.95076345691556e-17
36 9.95076345691556e-17
37 9.95076345691556e-17
38 9.95076345691556e-17
39 9.95076345691556e-17
40 9.95076345691556e-17
41 9.95076345691556e-17
42 9.95076345691556e-17
43 9.95076345691556e-17
44 9.95076345691556e-17
45 9.95076345691556e-17
46 9.95076345691556e-17
47 9.95076345691556e-17
48 9.95076345691556e-17
49 3.0416184978568e-17
};
\addlegendentry{$X^\phi_{ij}=\phi(x_i,t_j)$}
\end{axis}

\end{tikzpicture}

==> arxiv_version/images/tikz/smoothed_phiv2.tex <==
% This file was created by matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
%
\begin{tikzpicture}

\begin{axis}[%
width=0.262\figurewidth,
height=\figureheight,
at={(0.689\figurewidth,0\figureheight)},
scale only axis,
xmin=0,
xmax=20,
xlabel style={font=\color{white!15!black}},
xlabel={$n$ modes},
ymode=log,
ymin=1e-17,
ymax=1,
yminorticks=true,
axis background/.style={fill=white},
title style={font=\bfseries},
title={paraboloid},
legend style={at={(0.97,0.5)}, anchor=east, legend cell align=left, align=left, fill=none, draw=none},
scaled ticks=false, xticklabel style={/pgf/number format/fixed},yticklabel style={/pgf/number format/fixed}
]
\addplot [color=black, line width=1.5pt]
  table[row sep=crcr]{%
0	1\\
1	0.108715760217601\\
2	0.108715634236489\\
3	0.0920641111130334\\
4	0.0920640847955109\\
5	0.068791913048795\\
6	0.0687918193595006\\
7	0.0447255749252609\\
8	0.044725562332172\\
9	0.0270961356129575\\
10	0.027096041422363\\
11	0.0229775396649234\\
12	0.0229774237831645\\
13	0.0219687207092515\\
14	0.0219685229489843\\
15	0.0214905919511001\\
16	0.0214903863358998\\
17	0.0169406684748452\\
18	0.0169404955096078\\
19	0.0125606794962384\\
20	0.0125602504887935\\
21	0.012095808160281\\
22	0.012095753375457\\
23	0.0114919120191121\\
24	0.0114915874902618\\
25	0.0114791822764769\\
26	0.0114791164300901\\
27	0.00942848486431508\\
28	0.00942818463158277\\
29	0.00753288540033795\\
30	0.00753278297038982\\
31	0.00752777202203293\\
32	0.0075272738516459\\
33	0.00720851011526472\\
34	0.00720817840874839\\
35	0.00712811894643316\\
36	0.00712798767233169\\
37	0.00598874820673185\\
38	0.00598869108086194\\
39	0.0051289427089822\\
40	0.00512891965034824\\
41	0.00503424481958879\\
42	0.00503424452216082\\
43	0.00494515674123981\\
44	0.00494492780082036\\
45	0.00487137514777922\\
46	0.00487037432500624\\
47	0.00421444940822556\\
48	0.00421409967359719\\
49	0.00395873561982647\\
50	0.00395846526079949\\
51	0.00386362980513069\\
52	0.00386353684236286\\
53	0.00377082854130412\\
54	0.00377030557373398\\
55	0.00372967042540982\\
56	0.00372896245992916\\
57	0.00351333695898237\\
58	0.00351271540544044\\
59	0.00330378411420591\\
};
\addlegendentry{$\frac{\Vert q - q_n\Vert}{\Vert q \Vert}$}

\addplot [color=mycolor1, dashed]
  table[row sep=crcr]{%
0	1\\
1	0.436930895045629\\
2	0.436887632419151\\
3	3.8193175378319e-16\\
4	3.61094984130645e-16\\
5	1.96856041779954e-16\\
6	1.54143069352301e-16\\
7	1.05611075450375e-16\\
8	8.67295662566665e-17\\
9	8.67295662566665e-17\\
10	8.67295662566665e-17\\
11	8.67295662566665e-17\\
12	8.67295662566665e-17\\
13	8.67295662566665e-17\\
14	8.67295662566665e-17\\
15	8.67295662566665e-17\\
16	8.67295662566665e-17\\
17	8.67295662566665e-17\\
18	8.67295662566665e-17\\
19	8.67295662566665e-17\\
20	8.67295662566665e-17\\
21	8.67295662566665e-17\\
22	8.67295662566665e-17\\
23	8.67295662566665e-17\\
24	8.67295662566665e-17\\
25	8.67295662566665e-17\\
26	8.67295662566665e-17\\
27	8.67295662566665e-17\\
28	8.67295662566665e-17\\
29	8.67295662566665e-17\\
30	8.67295662566665e-17\\
31	8.67295662566665e-17\\
32	8.67295662566665e-17\\
33	8.67295662566665e-17\\
34	8.67295662566665e-17\\
35	8.67295662566665e-17\\
36	8.67295662566665e-17\\
37	8.67295662566665e-17\\
38	8.67295662566665e-17\\
39	8.67295662566665e-17\\
40	8.67295662566665e-17\\
41	8.67295662566665e-17\\
42	8.67295662566665e-17\\
43	8.67295662566665e-17\\
44	8.67295662566665e-17\\
45	8.67295662566665e-17\\
46	8.67295662566665e-17\\
47	8.67295662566665e-17\\
48	8.67295662566665e-17\\
49	8.67295662566665e-17\\
50	8.67295662566665e-17\\
51	8.67295662566665e-17\\
52	8.67295662566665e-17\\
53	8.67295662566665e-17\\
54	8.67295662566665e-17\\
55	8.67295662566665e-17\\
56	8.67295662566665e-17\\
57	8.67295662566665e-17\\
58	5.12180668652929e-17\\
59	1.62766191257076e-17\\
};
\addlegendentry{$ \frac{\Vert\varphi-\varphi_n\Vert}{\Vert \varphi \Vert}$}

\addplot [color=black!30!mycolor1, mark size=0.8pt, mark=*, mark options={solid, fill=mycolor1, black!30!mycolor1}]
  table[row sep=crcr]{%
0	1\\
1	0.114746569351737\\
2	0.108715634236489\\
3	0.000394256743858815\\
4	0.000394256743858815\\
5	0.000394256743858814\\
6	0.000394256743858814\\
7	0.000394256743858813\\
8	0.000394256743858813\\
9	0.000394256743858811\\
10	0.000394256743858811\\
11	0.000394256743858808\\
12	0.000394256743858809\\
13	0.000394256743858809\\
14	0.000394256743858807\\
15	0.000394256743858802\\
16	0.000394256743858802\\
17	0.0003942567438588\\
18	0.000394256743858801\\
19	0.000394256743858801\\
20	0.0003942567438588\\
21	0.000394256743858799\\
22	0.000394256743858797\\
23	0.000394256743858796\\
24	0.000394256743858795\\
25	0.000394256743858796\\
26	0.000394256743858795\\
27	0.000394256743858796\\
28	0.000394256743858796\\
29	0.000394256743858793\\
30	0.000394256743858792\\
31	0.000394256743858791\\
32	0.000394256743858791\\
33	0.000394256743858791\\
34	0.000394256743858792\\
35	0.000394256743858792\\
36	0.000394256743858792\\
37	0.000394256743858792\\
38	0.000394256743858794\\
39	0.000394256743858794\\
40	0.000394256743858793\\
41	0.000394256743858794\\
42	0.000394256743858794\\
43	0.000394256743858794\\
44	0.000394256743858793\\
45	0.000394256743858794\\
46	0.000394256743858794\\
47	0.000394256743858794\\
48	0.000394256743858794\\
49	0.000394256743858794\\
50	0.000394256743858793\\
51	0.000394256743858793\\
52	0.000394256743858793\\
53	0.000394256743858794\\
54	0.000394256743858794\\
55	0.000394256743858795\\
56	0.000394256743858796\\
57	0.000394256743858796\\
58	0.000394256743858797\\
59	0.000394256743858797\\
};
\addlegendentry{$\frac{\Vert q - f(\varphi_n)\Vert}{\Vert q \Vert}$}

\end{axis}

\begin{axis}[%
width=0.262\figurewidth,
height=\figureheight,
at={(0.345\figurewidth,0\figureheight)},
scale only axis,
xmin=0,
xmax=20,
xlabel style={font=\color{white!15!black}},
xlabel={$n$ modes},
ymode=log,
ymin=0.0005,
ymax=1,
yminorticks=true,
axis background/.style={fill=white},
title style={font=\bfseries},
title={signed distance},
legend style={legend cell align=left, align=left, fill=none, draw=none},
scaled ticks=false, xticklabel style={/pgf/number format/fixed},yticklabel style={/pgf/number format/fixed}
]
\addplot [color=black, line width=1.5pt]
  table[row sep=crcr]{%
0	1\\
1	0.108715760217601\\
2	0.108715634236489\\
3	0.0920641111130334\\
4	0.0920640847955109\\
5	0.068791913048795\\
6	0.0687918193595006\\
7	0.0447255749252609\\
8	0.044725562332172\\
9	0.0270961356129575\\
10	0.027096041422363\\
11	0.0229775396649234\\
12	0.0229774237831645\\
13	0.0219687207092515\\
14	0.0219685229489843\\
15	0.0214905919511001\\
16	0.0214903863358998\\
17	0.0169406684748452\\
18	0.0169404955096078\\
19	0.0125606794962384\\
20	0.0125602504887935\\
21	0.012095808160281\\
22	0.012095753375457\\
23	0.0114919120191121\\
24	0.0114915874902618\\
25	0.0114791822764769\\
26	0.0114791164300901\\
27	0.00942848486431508\\
28	0.00942818463158277\\
29	0.00753288540033795\\
30	0.00753278297038982\\
31	0.00752777202203293\\
32	0.0075272738516459\\
33	0.00720851011526472\\
34	0.00720817840874839\\
35	0.00712811894643316\\
36	0.00712798767233169\\
37	0.00598874820673185\\
38	0.00598869108086194\\
39	0.0051289427089822\\
40	0.00512891965034824\\
41	0.00503424481958879\\
42	0.00503424452216082\\
43	0.00494515674123981\\
44	0.00494492780082036\\
45	0.00487137514777922\\
46	0.00487037432500624\\
47	0.00421444940822556\\
48	0.00421409967359719\\
49	0.00395873561982647\\
50	0.00395846526079949\\
51	0.00386362980513069\\
52	0.00386353684236286\\
53	0.00377082854130412\\
54	0.00377030557373398\\
55	0.00372967042540982\\
56	0.00372896245992916\\
57	0.00351333695898237\\
58	0.00351271540544044\\
59	0.00330378411420591\\
};
\addlegendentry{$\frac{\Vert q - q_n\Vert}{\Vert q \Vert}$}

\addplot [color=mycolor2, dashed]
  table[row sep=crcr]{%
0	1\\
1	0.359805938935254\\
2	0.359781909976563\\
3	0.0545753225224157\\
4	0.0500049248468868\\
5	0.0171580345029261\\
6	0.017158024593463\\
7	0.00779911962046153\\
8	0.00778353165319985\\
9	0.0042627190538161\\
10	0.00426251172388405\\
11	0.00262415547666798\\
12	0.00262415415631536\\
13	0.00175172931821419\\
14	0.00175156803775569\\
15	0.00123912298873581\\
16	0.00123892084453071\\
17	0.000915256610565958\\
18	0.00091516079845879\\
19	0.000699140233566558\\
20	0.000699045948601238\\
21	0.000548607680110321\\
22	0.000548416146416228\\
23	0.000440031206785236\\
24	0.00043977995696157\\
25	0.000359558164702627\\
26	0.000359091518308983\\
27	0.000298257186097594\\
28	0.000297968409405683\\
29	0.000250882821298186\\
30	0.000250481873870689\\
31	0.000213482323544853\\
32	0.000213133469577126\\
33	0.000183854730360781\\
34	0.000183005373762078\\
35	0.000159403599160049\\
36	0.000159116464151412\\
37	0.000139579794036746\\
38	0.00013945920984066\\
39	0.000123354637878814\\
40	0.000123184854554119\\
41	0.000109956893484961\\
42	0.000109689916688902\\
43	9.88863166128095e-05\\
44	9.84504105634589e-05\\
45	8.96135256736368e-05\\
46	8.92384571188144e-05\\
47	8.18505811983025e-05\\
48	8.17956139497048e-05\\
49	7.59996218074654e-05\\
50	7.52597664068509e-05\\
51	7.07158604120756e-05\\
52	7.07106337064115e-05\\
53	6.70454953857494e-05\\
54	6.69344981723225e-05\\
55	6.44948263828488e-05\\
56	6.42298844051814e-05\\
57	6.28061113603602e-05\\
58	6.27910691174383e-05\\
59	6.22824346975996e-05\\
};
\addlegendentry{$ \frac{\Vert\phi-\phi_n\Vert}{\Vert \phi \Vert}$}

\addplot [color=black!30!mycolor2, mark size=0.8pt, mark=*, mark options={solid, fill=mycolor2, black!30!mycolor2}]
  table[row sep=crcr]{%
0	1\\
1	0.114746569346325\\
2	0.108715634236489\\
3	0.0450522534038761\\
4	0.0374498941113154\\
5	0.0181735389760626\\
6	0.0146773480144537\\
7	0.00978676663765104\\
8	0.00783460523447255\\
9	0.00502331305582069\\
10	0.00418318670877018\\
11	0.00215837737150043\\
12	0.00181254054959292\\
13	0.00119371870838012\\
14	0.00124273657563884\\
15	0.0013592880812847\\
16	0.00130839543498418\\
17	0.00126335206939511\\
18	0.00107346853540631\\
19	0.0008359911810919\\
20	0.000660255431805165\\
21	0.000369286463864993\\
22	0.000334743045209134\\
23	0.000307987996633321\\
24	0.000356998703881149\\
25	0.000414889000216105\\
26	0.000398806602529724\\
27	0.000385282073182484\\
28	0.00032799906449284\\
29	0.00025515368600473\\
30	0.00021397382639723\\
31	0.000137710698600638\\
32	0.000119900079294296\\
33	0.000148214466374314\\
34	0.000162383477899913\\
35	0.000174876144600143\\
36	0.000164410209801904\\
37	0.000162608212125621\\
38	0.000142256243929035\\
39	0.000111834274284489\\
40	9.22647874621909e-05\\
41	7.65407876379624e-05\\
42	7.59304873291416e-05\\
43	0.000100163528522023\\
44	0.000110763683328318\\
45	0.000120706775731265\\
46	0.000108558129344227\\
47	9.53491419425109e-05\\
48	7.46230170551248e-05\\
49	5.01243240728103e-05\\
50	4.66349602546242e-05\\
51	3.38326534582241e-05\\
52	5.85898716148313e-05\\
53	7.66496277901862e-05\\
54	8.57677161740406e-05\\
55	9.4280784157448e-05\\
56	8.54197595429984e-05\\
57	7.60067300788018e-05\\
58	5.93422600159246e-05\\
59	2.91370772041188e-05\\
};
\addlegendentry{$\frac{\Vert q - f(\phi_n)\Vert}{\Vert q \Vert}$}

\end{axis}

\begin{axis}[%
width=0.262\figurewidth,
height=\figureheight,
at={(0\figurewidth,0\figureheight)},
scale only axis,
xmin=0,
xmax=1,
xlabel style={font=\color{white!15!black}},
xlabel={$x$},
ymin=-0.2,
ymax=0.5,
axis background/.style={fill=white},
title style={font=\bfseries},
title={levelset function},
scaled ticks=false, xticklabel style={/pgf/number format/fixed},yticklabel style={/pgf/number format/fixed}
]
\addplot [color=mycolor1, dashed, forget plot]
  table[row sep=crcr]{%
0	0.847721129991393\\
0.01	0.812978988936933\\
0.02	0.778903514549138\\
0.03	0.745494706828011\\
0.04	0.71275256577355\\
0.05	0.680677091385756\\
0.06	0.649268283664628\\
0.07	0.618526142610167\\
0.08	0.588450668222373\\
0.09	0.559041860501246\\
0.1	0.530299719446785\\
0.11	0.50222424505899\\
0.12	0.474815437337863\\
0.13	0.448073296283402\\
0.14	0.421997821895608\\
0.15	0.39658901417448\\
0.16	0.371846873120019\\
0.17	0.347771398732225\\
0.18	0.324362591011097\\
0.19	0.301620449956637\\
0.2	0.279544975568842\\
0.21	0.258136167847715\\
0.22	0.237394026793254\\
0.23	0.21731855240546\\
0.24	0.197909744684332\\
0.25	0.179167603629871\\
0.26	0.161092129242077\\
0.27	0.143683321520949\\
0.28	0.126941180466489\\
0.29	0.110865706078694\\
0.3	0.0954568983575668\\
0.31	0.0807147573031059\\
0.32	0.0666392829153116\\
0.33	0.0532304751941841\\
0.34	0.0404883341397232\\
0.35	0.028412859751929\\
0.36	0.0170040520308014\\
0.37	0.00626191097634053\\
0.38	-0.00381356341145371\\
0.39	-0.0132223711325813\\
0.4	-0.0219645121870422\\
0.41	-0.0300399865748363\\
0.42	-0.0374487942959639\\
0.43	-0.0441909353504248\\
0.44	-0.050266409738219\\
0.45	-0.0556752174593466\\
0.46	-0.0604173585138075\\
0.47	-0.0644928329016017\\
0.48	-0.0679016406227292\\
0.49	-0.0706437816771901\\
0.5	-0.0727192560649844\\
0.51	-0.0741280637861119\\
0.52	-0.0748702048405728\\
0.53	-0.074945679228367\\
0.54	-0.0743544869494946\\
0.55	-0.0730966280039555\\
0.56	-0.0711721023917497\\
0.57	-0.0685809101128773\\
0.58	-0.0653230511673382\\
0.59	-0.0613985255551324\\
0.6	-0.0568073332762599\\
0.61	-0.0515494743307208\\
0.62	-0.045624948718515\\
0.63	-0.0390337564396426\\
0.64	-0.0317758974941035\\
0.65	-0.0238513718818977\\
0.66	-0.0152601796030252\\
0.67	-0.00600232065748609\\
0.68	0.0039222049547197\\
0.69	0.014513397233592\\
0.7	0.0257712561791312\\
0.71	0.0376957817913369\\
0.72	0.0502869740702094\\
0.73	0.0635448330157485\\
0.74	0.0774693586279543\\
0.75	0.0920605509068268\\
0.76	0.107318409852366\\
0.77	0.123242935464572\\
0.78	0.139834127743444\\
0.79	0.157091986688983\\
0.8	0.175016512301189\\
0.81	0.193607704580062\\
0.82	0.2128655635256\\
0.83	0.232790089137806\\
0.84	0.253381281416679\\
0.85	0.274639140362218\\
0.86	0.296563665974424\\
0.87	0.319154858253296\\
0.88	0.342412717198835\\
0.89	0.366337242811041\\
0.9	0.390928435089914\\
0.91	0.416186294035453\\
0.92	0.442110819647659\\
0.93	0.468702011926531\\
0.94	0.49595987087207\\
0.95	0.523884396484276\\
0.96	0.552475588763148\\
0.97	0.581733447708687\\
0.98	0.611657973320893\\
0.99	0.642249165599766\\
1	0.673507024545305\\
};
\addplot [color=mycolor2, forget plot]
  table[row sep=crcr]{%
0	0.376133385176628\\
0.01	0.366133409770264\\
0.02	0.356133435335724\\
0.03	0.34613346193177\\
0.04	0.336133489622002\\
0.05	0.326133518475361\\
0.06	0.316133548566705\\
0.07	0.306133579977456\\
0.08	0.296133612796337\\
0.09	0.286133647120208\\
0.1	0.276133683055019\\
0.11	0.266133720716907\\
0.12	0.256133760233447\\
0.13	0.246133801745093\\
0.14	0.236133845406851\\
0.15	0.226133891390212\\
0.16	0.2161339398854\\
0.17	0.206133991104005\\
0.18	0.196134045282069\\
0.19	0.186134102683722\\
0.2	0.17613416360549\\
0.21	0.166134228381418\\
0.22	0.156134297389195\\
0.23	0.146134371057528\\
0.24	0.136134449875054\\
0.25	0.126134534401189\\
0.26	0.116134625279431\\
0.27	0.106134723253769\\
0.28	0.0961348291890982\\
0.29	0.08613494409682\\
0.3	0.0761350691672347\\
0.31	0.066135205810927\\
0.32	0.0561353557121958\\
0.33	0.0461355208988296\\
0.34	0.0361357038343717\\
0.35	0.0261359075418147\\
0.36	0.0161361357719639\\
0.37	0.00613639323649742\\
0.38	-0.00386331406329249\\
0.39	-0.0138629783628802\\
0.4	-0.0238625894356185\\
0.41	-0.0338621335328176\\
0.42	-0.0438615917247162\\
0.43	-0.0538609372061878\\
0.44	-0.0638601307260436\\
0.45	-0.0738591124152337\\
0.46	-0.0838577862038338\\
0.47	-0.093855987589775\\
0.48	-0.103853409517265\\
0.49	-0.113849405304436\\
0.5	-0.123842339926807\\
0.51	-0.133826538275112\\
0.52	-0.143759924052693\\
0.53	-0.14596314088803\\
0.54	-0.136084040990588\\
0.55	-0.126104151012919\\
0.56	-0.116112402232157\\
0.57	-0.106116894297044\\
0.58	-0.0961197192861938\\
0.59	-0.0861216599036865\\
0.6	-0.0761230752052982\\
0.61	-0.0661241530547455\\
0.62	-0.056125001281249\\
0.63	-0.0461256861966962\\
0.64	-0.0361262508223736\\
0.65	-0.0261267242887688\\
0.66	-0.0161271270230879\\
0.67	-0.00612747377364165\\
0.68	0.0038722245449643\\
0.69	0.0138719596821787\\
0.7	0.023871725285451\\
0.71	0.0338715163841346\\
0.72	0.0438713290331059\\
0.73	0.0538711600612616\\
0.74	0.0638710068905701\\
0.75	0.0738708674036174\\
0.76	0.0838707398451328\\
0.77	0.093870622747742\\
0.78	0.103870514875267\\
0.79	0.113870415178919\\
0.8	0.123870322763086\\
0.81	0.133870236858355\\
0.82	0.14387015680004\\
0.83	0.153870082010951\\
0.84	0.163870011987453\\
0.85	0.173869946288113\\
0.86	0.183869884524386\\
0.87	0.193869826352922\\
0.88	0.203869771469181\\
0.89	0.213869719602102\\
0.9	0.223869670509623\\
0.91	0.233869623974906\\
0.92	0.243869579803134\\
0.93	0.253869537818785\\
0.94	0.263869497863301\\
0.95	0.273869459793086\\
0.96	0.283869423477784\\
0.97	0.293869388798784\\
0.98	0.303869355647931\\
0.99	0.313869323926394\\
1	0.323869293543685\\
};
\end{axis}
\end{tikzpicture}%


==> arxiv_version/myshortcuts.tex <==
% ############################################################################
% 	My math shortcuts
% ############################################################################
\usepackage{amsmath,amssymb,mathtools}
%#####################
% 1. Model reduction
%####################
% singular value functional
\newcommand{\Jsigma}{\mathcal{J}}

%####################
% 2. General Math
%####################
\newcommand{\defeq}{\coloneqq}
\renewcommand{\vec}[1]{\mathbf{#1}}
\newcommand{\matr}[1]{\mathbf{#1}}
\newcommand{\tran}[1]{#1^{\intercal}}
\newcommand{\abs}[1]{\left | #1 \right |}
\newcommand{\ord}[1]{\mathcal{O}\left( #1 \right) }
\newcommand{\tr}[1]{\mathrm{tr}\left( #1 \right) }
\renewcommand{\vec}[1]{\mathbf{#1}}
\newcommand{\norm}[1]{\left\Vert #1 \right\Vert}
\newcommand{\Res}{\mathcal{R}}
%####################
% 3. Derivatives 
%####################
\newcommand{\pd}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\td}[2]{\frac{\mathrm{d} #1}{\mathrm{d} #2}}
\renewcommand{\d}[1]{\mathrm{d}#1\;}

%####################
% 4. levelset function
%####################
\newcommand{\levelCurve}{\mathcal{C}}
\newcommand{\segCurve}{{\levelCurve_0}}

%####################
%  5. grid data
%####################
\newcommand{\mesh}{\Omega}

%####################
% 6. other
%####################
\newcommand{\x}{\vec{x}}
\newcommand{\highlight}[1]{{\color{blue}#1}}


